Sensitive 3mm Imaging of Discrete Sources in the Fields of tSZ-Selected Galaxy Clusters

In this paper we present the results of a blind survey for compact sources in 243 Galaxy clusters that were identified using the thermal Sunyaev-Zeldovich effect (tSZ). The survey was carried out at 90 GHz using MUSTANG2 on the Green Bank telescope and achieved a $5\sigma$ detection limit of 1 mJy in the center of each cluster. We detected 24 discrete sources. The majority (18) of these correspond to known radio sources, and of these, 5 show signs of significant variability, either with time or in spectral index. The remaining sources have no clear counterparts at other wavelengths. Searches for galaxy clusters via the tSZ effect strongly rely on observations at 90 GHz, and the sources found have the potential to bias mass estimates of clusters. We compare our results to the simulation Websky that can be used to estimate the source contamination in galaxy cluster catalogs. While the simulation showed a good match to our observations at the clusters' centers, it does not match our source distribution further out. Sources over 104" from a cluster's center bias the tSZ signal high, for some of our sources, by over 50%. When averaged over the whole cluster population the effect is smaller but still at a level of 1 to 2%. We also discovered that unlike previous measurements and simulations we see an enhancement of source counts in the outer regions of the clusters and fewer sources than expected in the centers of this tSZ selected sample.

==> fig4_figset.tex <==
\figsetstart
\figsetnum{4}
\figsettitle{SNR maps of M2-ACT sources and their counterparts in other surveys}

\figsetgrpstart
\figsetgrpnum{4.1}
\figsetgrptitle{Source 1:M2-SJ0201.8$-$0212}
\includegraphics[width=0.45\linewidth]{Source_1_snr_all_src_M2-SJ0201.8_-_0212.png}
\includegraphics[width=0.45\linewidth]{SED_Source_1_snr_all_src_M2-SJ0201.8_-_0212.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.2}
\figsetgrptitle{Source 2:M2-SJ0201.7$-$0212}
\includegraphics[width=0.45\linewidth]{Source_2_snr_all_src_M2-SJ0201.7_-_0212.png}
\includegraphics[width=0.45\linewidth]{SED_Source_2_snr_all_src_M2-SJ0201.7_-_0212.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.3}
\figsetgrptitle{Source 3:M2-SJ0204.5$+$0320}
\includegraphics[width=0.45\linewidth]{Source_3_snr_all_src_M2-SJ0204.5_+_0320.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_3_snr_all_src_M2-SJ0204.5_+_0320.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.4}
\figsetgrptitle{Source 4:M2-SJ0208.5$-$0259}
\includegraphics[width=0.45\linewidth]{Source_4_snr_all_src_M2-SJ0208.5_-_0259.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_4_snr_all_src_M2-SJ0208.5_-_0259.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.5}
\figsetgrptitle{Source 4:M2-SJ0220.8$-$0333}
\includegraphics[width=0.45\linewidth]{Source_5_snr_all_src_M2-SJ0220.8_-_0333.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_5_snr_all_src_M2-SJ0220.8_-_0333.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.6}
\figsetgrptitle{Source 6:M2-SJ0223.7$+$0019}
\includegraphics[width=0.45\linewidth]{Source_6_snr_all_src_M2-SJ0223.7_+_0019.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_6_snr_all_src_M2-SJ0223.7_+_0019.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.7}
\figsetgrptitle{Source 7:M2-SJ0231.7$-$0453}
      \includegraphics[width=0.45\linewidth]{Source_7_snr_all_src_M2-SJ0231.7_-_0453.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_7_snr_all_src_M2-SJ0231.7_-_0453.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.8}
\figsetgrptitle{Source 8:M2-SJ0233.3$+$0446}
  \includegraphics[width=0.45\linewidth]{Source_8_snr_all_src_M2-SJ0233.3_+_0446.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_8_snr_all_src_M2-SJ0233.3_+_0446.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.9}
\figsetgrptitle{Source 9:M2-SJ0248.1$-$0332}
   \includegraphics[width=0.45\linewidth]{Source_9_snr_all_src_M2-SJ0248.1_-_0332.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_9_snr_all_src_M2-SJ0248.1_-_0332.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.10}
\figsetgrptitle{Source 10:M2-SJ0248.4$-$0334}
 \includegraphics[width=0.45\linewidth]{Source_10_snr_all_src_M2-SJ0248.4_-_0334.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_10_snr_all_src_M2-SJ0248.4_-_0334.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.11}
\figsetgrptitle{Source 11:M2-SJ0249.6$+$0212}
 \includegraphics[width=0.45\linewidth]{Source_11_snr_all_src_M2-SJ0249.6_+_0212.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_11_snr_all_src_M2-SJ0249.6_+_0212.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.12}
\figsetgrptitle{Source 12:M2-SJ0839.7$-$0153}
     \includegraphics[width=0.45\linewidth]{Source_12_snr_all_src_M2-SJ0839.7_-_0153.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_12_snr_all_src_M2-SJ0839.7_-_0153.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.13}
\figsetgrptitle{Source 13:M2-SJ0839.7$-$0150}
  \includegraphics[width=0.45\linewidth]{Source_13_snr_all_src_M2-SJ0839.7_-_0150.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_13_snr_all_src_M2-SJ0839.7_-_0150.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.14}
\figsetgrptitle{Source 14:M2-SJ0901.4$+$0259}
 \includegraphics[width=0.45\linewidth]{Source_14_snr_all_src_M2-SJ0901.4_+_0259.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_14_snr_all_src_M2-SJ0901.4_+_0259.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.15}
\figsetgrptitle{Source 15:M2-SJ0905.7$+$0434}
    \includegraphics[width=0.45\linewidth]{Source_15_snr_all_src_M2-SJ0905.7_+_0434.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_15_snr_all_src_M2-SJ0905.7_+_0434.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.16}
\figsetgrptitle{Source 16:M2-SJ0918.8$+$0213}
 \includegraphics[width=0.45\linewidth]{Source_16_snr_all_src_M2-SJ0918.8_+_0213.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_16_snr_all_src_M2-SJ0918.8_+_0213.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.17}
\figsetgrptitle{Source 17:M2-SJ1118.0$-$0211}
 \includegraphics[width=0.45\linewidth]{Source_17_snr_all_src_M2-SJ1118.0_-_0211.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_17_snr_all_src_M2-SJ1118.0_-_0211.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.18}
\figsetgrptitle{Source 18:M2-SJ1148.2$-$0236}
 \includegraphics[width=0.45\linewidth]{Source_18_snr_all_src_M2-SJ1148.2_-_0236.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_18_snr_all_src_M2-SJ1148.2_-_0236.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.19}
\figsetgrptitle{Source 19:M2-SJ1152.4$+$0029}
\includegraphics[width=0.45\linewidth]{Source_19_snr_all_src_M2-SJ1152.4_+_0029.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_19_snr_all_src_M2-SJ1152.4_+_0029.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.20}
\figsetgrptitle{Source 20:M2-SJ1204.0$+$0127}
\includegraphics[width=0.45\linewidth]{Source_20_snr_all_src_M2-SJ1204.0_+_0127.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_20_snr_all_src_M2-SJ1204.0_+_0127.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.21}
\figsetgrptitle{Source 21:M2-SJ1210.3$+$0224}
\includegraphics[width=0.45\linewidth]{Source_21_snr_all_src_M2-SJ1210.3_+_0224.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_21_snr_all_src_M2-SJ1210.3_+_0224.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.22}
\figsetgrptitle{Source 22:M2-SJ1220.3$-$0241}
\includegraphics[width=0.45\linewidth]{Source_22_snr_all_src_M2-SJ1220.3_-_0241.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_22_snr_all_src_M2-SJ1220.3_-_0241.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.23}
\figsetgrptitle{Source 23:M2-SJ1224.5$+$0211}
  \includegraphics[width=0.45\linewidth]{Source_23_snr_all_src_M2-SJ1224.5_+_0211.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_23_snr_all_src_M2-SJ1224.5_+_0211.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{4.24}
\figsetgrptitle{Source 24:M2-SJ1401.0$+$0252}
 \includegraphics[width=0.45\linewidth]{Source_24_snr_all_src_M2-SJ1401.0_+_0252.png}
    \includegraphics[width=0.45\linewidth]{SED_Source_24_snr_all_src_M2-SJ1401.0_+_0252.png}
\figsetgrpnote{\figfourcaption}
\figsetgrpend

\figsetend  


==> tab1.tex <==
%ACT DR5 name & map noise (mJy/beam) & M500c ($\times10^{14}M_\odot$) & $y_c\times 10^{-4}$ & redshift \\
\clearpage
\renewcommand{\thetable}{1}
\startlongtable
\begin{deluxetable}{ccccc}
%\captionsetup{labelformat=empty}
\tablecaption{On-line extra: A list of ACT DR5 clusters with successful observations and the depth of each map.  Individual maps can be found on dataverse (\url{https://dataverse.harvard.edu})}
%\hline
 %\begin{center} 
%\begin{scriptsize}
%\hspace{-1.3cm}\resizebox{1.2\linewidth}{!}{%
\tablehead{\colhead{ACT} & \colhead{map noise} & \colhead{M500c} & 
\colhead{Compton-$y$ ($y_c$)} & \colhead{redshift}  \\
\colhead{Cluster ID} &  \colhead{(mJy)}     & \colhead{($\times10^{14}\rm M_\odot$)}  & \colhead{($\times 10^{-4}$)} &
%        &  (mJy)     & ($\times10^{14}M_\odot$)  & ($\times 10^{-4}$) &
        }
\startdata
ACT-CLJ0200.3+0019 & 0.13 & 1.74 & 0.69 & 0.70 \\
ACT-CLJ0201.6-0211 & 0.17 & 2.85 & 0.63 & 0.20 \\
ACT-CLJ0201.6-0503 & 0.14 & 1.68 & 0.53 & 0.81 \\
ACT-CLJ0203.0-0042 & 0.16 & 1.95 & 0.46 & 0.44 \\
ACT-CLJ0203.2-0123 & 0.14 & 2.07 & 0.42 & 0.71 \\
ACT-CLJ0203.7+0216 & 0.14 & 1.86 & 0.44 & 0.35 \\
ACT-CLJ0203.9-0205 & 0.17 & 1.47 & 0.31 & 0.88 \\
ACT-CLJ0204.5+0321 & 0.15 & 1.67 & 0.51 & 0.47 \\
ACT-CLJ0204.7-0116 & 0.15 & 1.51 & 0.32 & 0.30 \\
ACT-CLJ0204.8-0303 & 0.17 & 3.28 & 1.22 & 0.55 \\
ACT-CLJ0205.2-0439 & 0.16 & 3.16 & 1.12 & 0.97 \\
ACT-CLJ0205.9-0307 & 0.16 & 1.96 & 0.54 & 0.49 \\
ACT-CLJ0206.2-0114 & 0.16 & 4.02 & 1.08 & 0.68 \\
ACT-CLJ0206.4-0118 & 0.16 & 1.64 & 0.55 & 0.20 \\
ACT-CLJ0206.9-0119 & 0.16 & 1.68 & 0.51 & 0.54 \\
ACT-CLJ0207.2+0536 & 0.15 & 2.56 & 0.58 & 0.25 \\
ACT-CLJ0207.7+0020 & 0.12 & 2.33 & 1.77 & 0.97 \\
ACT-CLJ0208.2-0237 & 0.12 & 1.95 & 0.94 & 0.59 \\
ACT-CLJ0208.3-0255 & 0.13 & 1.87 & 0.64 & 0.94 \\
ACT-CLJ0209.6+0222 & 0.13 & 2.85 & 0.63 & 0.41 \\
ACT-CLJ0209.9+0038 & 0.12 & 1.52 & 0.97 & 0.94 \\
ACT-CLJ0210.0-0243 & 0.14 & 1.57 & 0.60 & 0.90 \\
ACT-CLJ0210.1+0254 & 0.13 & 1.54 & 0.32 & 0.15 \\
ACT-CLJ0211.1-0453 & 0.14 & 1.56 & 0.62 & 0.14 \\
ACT-CLJ0211.2-0343 & 0.14 & 2.74 & 0.84 & 0.73 \\
ACT-CLJ0211.9-0146 & 0.14 & 1.71 & 0.33 & 0.60 \\
ACT-CLJ0212.5-0037 & 0.13 & 1.76 & 0.39 & 0.42 \\
ACT-CLJ0212.5+0152 & 0.14 & 1.98 & 0.43 & 0.87 \\
ACT-CLJ0214.7-0432 & 0.15 & 1.09 & 0.31 & 0.14 \\
ACT-CLJ0215.4+0030 & 0.13 & 3.49 & 1.80 & 0.86 \\
ACT-CLJ0215.4-0440 & 0.14 & 1.57 & 0.48 & 0.35 \\
ACT-CLJ0215.6-0113 & 0.14 & 1.97 & 0.99 & 0.93 \\
ACT-CLJ0215.8-0041 & 0.12 & 1.65 & 0.34 & 0.43 \\
ACT-CLJ0217.7-0345 & 0.13 & 1.38 & 0.65 & 1.91 \\
ACT-CLJ0217.8-0048 & 0.25 & 1.95 & 0.95 & 0.79 \\
ACT-CLJ0218.1-0214 & 0.22 & 1.60 & 0.49 & 1.16 \\
ACT-CLJ0218.2-0041 & 0.22 & 3.20 & 0.89 & 0.67 \\
ACT-CLJ0218.5-0114 & 0.23 & 1.94 & 0.68 & 0.90 \\
ACT-CLJ0218.7-0014 & 0.21 & 2.23 & 0.53 & 0.65 \\
ACT-CLJ0219.0+0303 & 0.19 & 1.65 & 0.53 & 0.48 \\
ACT-CLJ0219.8+0022 & 0.20 & 3.30 & 1.20 & 0.54 \\
ACT-CLJ0219.9+0130 & 0.18 & 2.94 & 0.70 & 0.37 \\
ACT-CLJ0219.9+0246 & 0.17 & 1.59 & 0.32 & 0.25 \\
ACT-CLJ0220.9-0332 & 0.19 & 1.64 & 0.46 & 1.03 \\
ACT-CLJ0221.6-0012 & 0.18 & 1.93 & 0.41 & 0.59 \\
ACT-CLJ0221.7-0346 & 0.19 & 3.11 & 0.82 & 0.43 \\
ACT-CLJ0221.9-0340 & 0.19 & 1.89 & 0.47 & 1.03 \\
ACT-CLJ0222.2+0520 & 0.18 & 2.12 & 0.45 & 0.81 \\
ACT-CLJ0223.1-0057 & 0.20 & 3.37 & 0.95 & 0.66 \\
ACT-CLJ0223.6+0020 & 0.19 & 1.63 & 0.32 & 0.59 \\
ACT-CLJ0224.5-0002 & 0.23 & 1.69 & 0.81 & 0.77 \\
ACT-CLJ0224.5+0102 & 0.20 & 2.10 & 0.72 & 0.83 \\
ACT-CLJ0225.4-0355 & 0.23 & 1.62 & 0.34 & 0.77 \\
ACT-CLJ0226.4+0426 & 0.15 & 2.44 & 1.23 & 0.49 \\
ACT-CLJ0227.6-0318 & 0.13 & 2.17 & 0.76 & 0.84 \\
ACT-CLJ0228.4+0030 & 0.14 & 2.06 & 0.44 & 0.73 \\
ACT-CLJ0229.6-0336 & 0.28 & 2.21 & 0.51 & 0.32 \\
ACT-CLJ0230.9+0248 & 0.23 & 1.92 & 0.44 & 0.25 \\
ACT-CLJ0231.7-0453 & 0.25 & 2.89 & 0.74 & 0.18 \\
ACT-CLJ0232.1+0230 & 0.23 & 1.80 & 0.39 & 0.62 \\
ACT-CLJ0232.7+0214 & 0.20 & 1.66 & 0.43 & 0.62 \\
ACT-CLJ0232.7+0350 & 0.21 & 2.24 & 0.93 & 0.57 \\
ACT-CLJ0233.2+0211 & 0.21 & 1.70 & 0.38 & 0.63 \\
ACT-CLJ0233.2+0248 & 0.21 & 1.74 & 0.46 & 0.50 \\
ACT-CLJ0233.2+0448 & 0.21 & 2.03 & 0.50 & 0.29 \\
ACT-CLJ0233.6-0530 & 0.22 & 2.84 & 0.73 & 0.43 \\
ACT-CLJ0233.7+0127 & 0.21 & 2.04 & 0.55 & 0.57 \\
ACT-CLJ0234.5-0107 & 0.23 & 2.08 & 0.56 & 0.54 \\
ACT-CLJ0234.6-0259 & 0.19 & 1.63 & 0.32 & 0.41 \\
ACT-CLJ0235.2-0323 & 0.10 & 1.73 & 0.35 & 0.58 \\
ACT-CLJ0235.5-0005 & 0.10 & 1.56 & 0.35 & 0.90 \\
ACT-CLJ0236.5+0106 & 0.10 & 1.79 & 0.57 & 0.79 \\
ACT-CLJ0236.7-0228 & 0.10 & 1.74 & 0.80 & 0.62 \\
ACT-CLJ0237.6-0423 & 0.10 & 1.72 & 0.39 & 0.45 \\
ACT-CLJ0238.1+0306 & 0.09 & 2.25 & 0.65 & 0.72 \\
ACT-CLJ0239.3-0332 & 0.08 & 2.16 & 0.77 & 0.25 \\
ACT-CLJ0239.8-0134 & 0.09 & 6.56 & 2.42 & 0.38 \\
ACT-CLJ0240.0+0116 & 0.08 & 3.71 & 0.99 & 0.60 \\
ACT-CLJ0240.0+0303 & 0.08 & 2.00 & 0.56 & 0.76 \\
ACT-CLJ0241.2-0018 & 0.08 & 3.09 & 1.80 & 0.69 \\
ACT-CLJ0241.4-0433 & 0.09 & 1.82 & 0.56 & 0.52 \\
ACT-CLJ0242.2-0345 & 0.09 & 1.87 & 0.57 & 1.10 \\
ACT-CLJ0242.7-0226 & 0.08 & 2.67 & 0.77 & 0.54 \\
ACT-CLJ0242.7-0450 & 0.08 & 1.57 & 1.05 & 0.48 \\
ACT-CLJ0242.9-0250 & 0.09 & 2.35 & 0.55 & 0.61 \\
ACT-CLJ0243.2+0256 & 0.09 & 2.05 & 0.60 & 0.95 \\
ACT-CLJ0245.2+0032 & 0.09 & 1.78 & 0.49 & 0.91 \\
ACT-CLJ0245.2-0240 & 0.14 & 1.90 & 1.29 & 1.08 \\
ACT-CLJ0245.2+0407 & 0.10 & 2.16 & 1.63 & 0.87 \\
ACT-CLJ0245.7-0028 & 0.15 & 1.89 & 0.50 & 0.58 \\
ACT-CLJ0245.8-0042 & 0.15 & 1.99 & 0.44 & 0.18 \\
ACT-CLJ0246.4+0429 & 0.17 & 2.21 & 0.98 & 0.42 \\
ACT-CLJ0247.3-0156 & 0.15 & 1.84 & 0.42 & 0.24 \\
ACT-CLJ0248.0-0331 & 0.14 & 3.52 & 0.81 & 0.19 \\
ACT-CLJ0248.2-0216 & 0.15 & 6.99 & 3.63 & 0.24 \\
ACT-CLJ0248.2+0238 & 0.15 & 4.83 & 2.14 & 0.55 \\
ACT-CLJ0248.3+0122 & 0.15 & 1.77 & 1.12 & 0.81 \\
ACT-CLJ0248.3-0337 & 0.14 & 1.51 & 1.10 & 0.18 \\
ACT-CLJ0248.7-0019 & 0.15 & 2.08 & 0.61 & 0.92 \\
ACT-CLJ0248.9-0328 & 0.16 & 2.48 & 0.87 & 0.67 \\
ACT-CLJ0249.6+0210 & 0.16 & 2.05 & 0.88 & 0.79 \\
ACT-CLJ0250.1+0008 & 0.16 & 3.15 & 1.53 & 0.84 \\
ACT-CLJ0253.5-0017 & 0.16 & 2.21 & 1.89 & 1.35 \\
ACT-CLJ0254.4-0538 & 0.18 & 2.32 & 1.81 & 0.97 \\
ACT-CLJ0256.5+0006 & 0.17 & 4.00 & 1.02 & 0.36 \\
ACT-CLJ0257.0-0300 & 0.15 & 2.03 & 0.40 & 0.66 \\
ACT-CLJ0258.4+0147 & 0.16 & 1.81 & 0.44 & 0.93 \\
ACT-CLJ0259.4-0524 & 0.15 & 1.95 & 0.43 & 0.84 \\
ACT-CLJ0259.8-0037 & 0.21 & 2.19 & 1.46 & 0.61 \\
ACT-CLJ0300.2+0125 & 0.21 & 2.87 & 1.40 & 1.27 \\
ACT-CLJ0301.5-0248 & 0.21 & 2.38 & 1.38 & 0.80 \\
ACT-CLJ0839.5-0140 & 0.15 & 2.59 & 0.62 & 0.26 \\
ACT-CLJ0839.5-0150 & 0.14 & 2.42 & 0.70 & 0.56 \\
ACT-CLJ0842.3+0033 & 0.14 & 1.97 & 1.61 & 1.03 \\
ACT-CLJ0842.9+0424 & 0.14 & 2.12 & 0.42 & 0.48 \\
ACT-CLJ0844.6+0216 & 0.15 & 2.53 & 0.52 & 0.57 \\
ACT-CLJ0845.0+0127 & 0.15 & 2.74 & 0.83 & 0.42 \\
ACT-CLJ0845.4+0327 & 0.15 & 4.75 & 1.22 & 0.33 \\
ACT-CLJ0848.4+0412 & 0.14 & 2.61 & 0.58 & 0.85 \\
ACT-CLJ0848.5-0122 & 0.15 & 2.40 & 0.50 & 0.61 \\
ACT-CLJ0849.6-0051 & 0.14 & 2.69 & 0.58 & 0.61 \\
ACT-CLJ0849.8+0440 & 0.16 & 2.44 & 0.71 & 0.74 \\
ACT-CLJ0852.2-0101 & 0.14 & 3.22 & 0.71 & 0.46 \\
ACT-CLJ0853.4+0132 & 0.15 & 2.02 & 1.57 & 0.49 \\
ACT-CLJ0854.7-0122 & 0.14 & 2.48 & 1.45 & 0.35 \\
ACT-CLJ0855.4-0106 & 0.15 & 2.69 & 1.58 & 0.75 \\
ACT-CLJ0856.3+0146 & 0.15 & 3.64 & 2.36 & 0.72 \\
ACT-CLJ0856.4-0013 & 0.15 & 2.25 & 1.71 & 0.42 \\
ACT-CLJ0856.5+0143 & 0.14 & 2.84 & 2.22 & 0.71 \\
ACT-CLJ0857.8+0310 & 0.14 & 4.58 & 1.20 & 0.20 \\
ACT-CLJ0859.0-0119 & 0.14 & 1.86 & 1.68 & 1.34 \\
ACT-CLJ0859.4+0308 & 0.15 & 1.81 & 0.39 & 0.19 \\
ACT-CLJ0901.5+0301 & 0.15 & 2.08 & 0.47 & 0.19 \\
ACT-CLJ0901.7+0408 & 0.16 & 2.13 & 0.76 & 0.85 \\
ACT-CLJ0903.4-0136 & 0.17 & 2.83 & 0.74 & 0.45 \\
ACT-CLJ0904.3+0206 & 0.17 & 2.35 & 0.72 & 0.81 \\
ACT-CLJ0904.5+0426 & 0.19 & 2.43 & 0.88 & 0.46 \\
ACT-CLJ0905.6+0434 & 0.23 & 1.81 & 0.40 & 0.24 \\
ACT-CLJ0907.8+0057 & 0.20 & 2.45 & 0.53 & 0.69 \\
ACT-CLJ0907.9+0254 & 0.21 & 2.06 & 0.43 & 0.81 \\
ACT-CLJ0909.5-0050 & 0.21 & 2.09 & 1.07 & 1.09 \\
ACT-CLJ0913.2+0349 & 0.16 & 2.99 & 0.71 & 0.46 \\
ACT-CLJ0914.7+0011 & 0.12 & 2.15 & 0.94 & 0.53 \\
ACT-CLJ0915.9-0132 & 0.13 & 2.76 & 1.02 & 0.49 \\
ACT-CLJ0916.1-0024 & 0.13 & 4.33 & 1.09 & 0.32 \\
ACT-CLJ0916.7+0155 & 0.14 & 2.35 & 1.95 & 1.15 \\
ACT-CLJ0916.8-0059 & 0.13 & 1.72 & 0.39 & 0.26 \\
ACT-CLJ0918.7+0211 & 0.12 & 2.11 & 0.44 & 0.28 \\
ACT-CLJ0920.4+0134 & 0.12 & 2.79 & 1.10 & 0.69 \\
ACT-CLJ0921.0-0148 & 0.13 & 2.15 & 0.46 & 0.59 \\
ACT-CLJ0921.3+0317 & 0.13 & 4.19 & 1.00 & 0.35 \\
ACT-CLJ0922.1-0027 & 0.13 & 2.99 & 0.80 & 0.32 \\
ACT-CLJ0922.1+0346 & 0.13 & 1.86 & 0.49 & 0.27 \\
ACT-CLJ0930.4+0216 & 0.11 & 4.11 & 1.14 & 0.54 \\
ACT-CLJ0935.0+0053 & 0.12 & 2.79 & 1.08 & 0.36 \\
ACT-CLJ0935.2+0048 & 0.12 & 5.31 & 1.40 & 0.36 \\
ACT-CLJ0935.3+0233 & 0.12 & 4.40 & 1.50 & 0.51 \\
ACT-CLJ0940.9+0322 & 0.12 & 1.96 & 1.37 & 0.49 \\
ACT-CLJ0943.7+0059 & 0.12 & 2.02 & 1.40 & 0.43 \\
ACT-CLJ0947.9-0120 & 0.13 & 4.05 & 3.88 & 1.10 \\
ACT-CLJ0951.6-0014 & 0.12 & 3.92 & 1.07 & 0.42 \\
ACT-CLJ0956.1+0158 & 0.12 & 2.51 & 0.80 & 0.95 \\
ACT-CLJ0957.6+0234 & 0.12 & 2.53 & 0.65 & 0.37 \\
ACT-CLJ1005.5+0235 & 0.13 & 2.04 & 0.42 & 0.37 \\
ACT-CLJ1006.9+0255 & 0.14 & 2.72 & 1.03 & 0.92 \\
ACT-CLJ1020.1-0013 & 0.10 & 1.95 & 1.27 & 0.40 \\
ACT-CLJ1020.3-0100 & 0.12 & 1.87 & 0.78 & 0.41 \\
ACT-CLJ1027.8+0004 & 0.15 & 2.33 & 1.32 & 0.71 \\
ACT-CLJ1029.9+0016 & 0.15 & 2.25 & 0.86 & 1.35 \\
ACT-CLJ1031.2+0031 & 0.13 & 2.22 & 1.62 & 0.88 \\
ACT-CLJ1032.1-0249 & 0.13 & 3.99 & 0.98 & 0.47 \\
ACT-CLJ1035.1-0248 & 0.14 & 3.77 & 1.24 & 0.58 \\
ACT-CLJ1035.1+0249 & 0.18 & 2.12 & 1.15 & 0.54 \\
ACT-CLJ1035.4-0001 & 0.13 & 2.86 & 1.31 & 0.48 \\
ACT-CLJ1036.2-0223 & 0.13 & 2.30 & 1.03 & 0.60 \\
ACT-CLJ1036.9+0154 & 0.24 & 2.09 & 0.49 & 0.60 \\
ACT-CLJ1049.3-0002 & 0.24 & 2.39 & 0.60 & 0.45 \\
ACT-CLJ1050.6+0017 & 0.25 & 3.17 & 1.55 & 0.59 \\
ACT-CLJ1053.7-0156 & 0.24 & 2.61 & 0.93 & 0.57 \\
ACT-CLJ1107.4+0121 & 0.14 & 2.52 & 0.57 & 0.61 \\
ACT-CLJ1110.2-0030 & 0.13 & 2.32 & 1.39 & 1.00 \\
ACT-CLJ1110.3+0143 & 0.13 & 2.76 & 0.67 & 0.62 \\
ACT-CLJ1110.8+0216 & 0.14 & 2.19 & 0.80 & 0.74 \\
ACT-CLJ1111.1+0044 & 0.13 & 2.44 & 0.54 & 0.18 \\
ACT-CLJ1112.8+0229 & 0.15 & 2.64 & 0.58 & 0.27 \\
ACT-CLJ1116.7+0218 & 0.15 & 1.76 & 0.37 & 0.48 \\
ACT-CLJ1116.9-0036 & 0.16 & 2.04 & 1.53 & 0.83 \\
ACT-CLJ1117.9-0211 & 0.16 & 2.62 & 0.59 & 0.45 \\
ACT-CLJ1118.7+0039 & 0.36 & 2.69 & 0.65 & 0.59 \\
ACT-CLJ1118.9-0041 & 0.56 & 1.90 & 1.46 & 0.24 \\
ACT-CLJ1125.7+0010 & 0.25 & 2.37 & 0.72 & 0.77 \\
ACT-CLJ1127.5+0003 & 0.28 & 1.53 & 0.39 & 1.36 \\
ACT-CLJ1128.3-0058 & 0.32 & 2.98 & 0.68 & 0.46 \\
ACT-CLJ1129.8+0256 & 0.33 & 2.58 & 0.60 & 0.23 \\
ACT-CLJ1131.6-0107 & 0.39 & 2.53 & 0.55 & 0.33 \\
ACT-CLJ1134.0+0116 & 0.39 & 2.29 & 1.63 & 0.73 \\
ACT-CLJ1136.9+0006 & 0.38 & 5.67 & 2.20 & 0.59 \\
ACT-CLJ1138.5-0011 & 0.47 & 2.20 & 0.67 & 0.88 \\
ACT-CLJ1139.3+0154 & 0.30 & 3.17 & 1.45 & 1.05 \\
ACT-CLJ1144.0+0440 & 0.13 & 1.86 & 0.41 & 0.41 \\
ACT-CLJ1144.2+0227 & 0.14 & 2.19 & 0.63 & 0.64 \\
ACT-CLJ1145.1-0100 & 0.11 & 1.76 & 0.38 & 0.70 \\
ACT-CLJ1148.0-0234 & 0.11 & 2.96 & 0.65 & 0.34 \\
ACT-CLJ1152.2+0031 & 0.14 & 3.58 & 0.80 & 0.46 \\
ACT-CLJ1152.5+0356 & 0.14 & 3.57 & 1.49 & 0.71 \\
ACT-CLJ1153.4+0259 & 0.14 & 2.33 & 1.32 & 0.70 \\
ACT-CLJ1154.2+0221 & 0.14 & 4.30 & 1.57 & 0.71 \\
ACT-CLJ1158.3+0228 & 0.12 & 3.57 & 2.20 & 0.48 \\
ACT-CLJ1158.9-0244 & 0.12 & 2.61 & 0.59 & 0.39 \\
ACT-CLJ1200.9-0125 & 0.12 & 2.03 & 0.62 & 0.25 \\
ACT-CLJ1202.8-0230 & 0.12 & 2.15 & 0.50 & 0.55 \\
ACT-CLJ1203.9+0126 & 0.15 & 3.27 & 0.76 & 0.41 \\
ACT-CLJ1205.3-0245 & 0.14 & 2.12 & 0.49 & 0.98 \\
ACT-CLJ1205.5+0214 & 0.13 & 1.96 & 1.38 & 0.77 \\
ACT-CLJ1208.3+0254 & 0.14 & 1.82 & 1.34 & 0.79 \\
ACT-CLJ1210.2+0223 & 0.13 & 2.66 & 0.56 & 0.38 \\
ACT-CLJ1210.2+0321 & 0.16 & 2.59 & 1.62 & 1.03 \\
ACT-CLJ1218.5+0233 & 0.13 & 3.74 & 1.11 & 0.77 \\
ACT-CLJ1220.4-0240 & 0.33 & 2.15 & 1.22 & 0.44 \\
ACT-CLJ1222.4-0127 & 0.15 & 2.53 & 0.59 & 0.29 \\
ACT-CLJ1222.6-0214 & 0.14 & 3.21 & 1.24 & 0.37 \\
ACT-CLJ1224.3+0211 & 0.51 & 2.12 & 0.45 & 0.45 \\
ACT-CLJ1238.5-0004 & 0.47 & 2.62 & 0.78 & 0.59 \\
ACT-CLJ1241.0+0010 & 0.29 & 2.22 & 0.54 & 0.79 \\
ACT-CLJ1245.0+0231 & 0.60 & 2.85 & 0.63 & 0.49 \\
ACT-CLJ1249.7+0145 & 0.68 & 1.94 & 1.50 & 0.16 \\
ACT-CLJ1250.6+0036 & 4.19 & 2.43 & 0.73 & 0.66 \\
ACT-CLJ1256.7+0235 & 0.34 & 3.54 & 1.14 & 0.51 \\
ACT-CLJ1258.4+0043 & 0.76 & 2.52 & 0.77 & 0.39 \\
ACT-CLJ1258.8+0059 & 0.41 & 2.21 & 0.66 & 0.39 \\
ACT-CLJ1301.2+0218 & 0.65 & 3.42 & 1.31 & 0.59 \\
ACT-CLJ1311.5-0119 & 0.68 & 9.98 & 8.85 & 0.20 \\
ACT-CLJ1315.0+0121 & 0.69 & 2.11 & 0.60 & 0.74 \\
ACT-CLJ1322.9-0227 & 0.97 & 2.94 & 0.96 & 0.79 \\
ACT-CLJ1324.9+0223 & 0.43 & 1.78 & 0.54 & 0.21 \\
ACT-CLJ1325.0+0209 & 0.33 & 2.26 & 0.64 & 0.64 \\
ACT-CLJ1326.8+0216 & 0.19 & 3.04 & 2.78 & 1.03 \\
ACT-CLJ1327.0+0212 & 0.18 & 4.60 & 1.15 & 0.26 \\
ACT-CLJ1328.4-0038 & 0.18 & 2.75 & 2.27 & 0.83 \\
ACT-CLJ1331.1+0100 & 0.17 & 4.63 & 1.37 & 0.35 \\
ACT-CLJ1332.8-0006 & 0.19 & 2.48 & 0.53 & 0.64 \\
ACT-CLJ1336.8-0104 & 0.18 & 1.86 & 1.46 & 0.43 \\
ACT-CLJ1340.9-0152 & 0.18 & 3.15 & 0.73 & 0.36 \\
ACT-CLJ1343.1-0000 & 0.21 & 2.64 & 1.25 & 0.72 \\
\enddata
\end{deluxetable}


